Correlated Time Series Forecasting using Deep Neural Networks: A Summary of Results

Cyber-physical systems often consist of entities that interact with each other over time. Meanwhile, as part of the continued digitization of industrial processes, various sensor technologies are deployed that enable us to record time-varying attributes (a.k.a., time series) of such entities, thus producing correlated time series. To enable accurate forecasting on such correlated time series, this paper proposes two models that combine convolutional neural networks (CNNs) and recurrent neural networks (RNNs). The first model employs a CNN on each individual time series, combines the convoluted features, and then applies an RNN on top of the convoluted features in the end to enable forecasting. The second model adds additional auto-encoders into the individual CNNs, making the second model a multi-task learning model, which provides accurate and robust forecasting. Experiments on two real-world correlated time series data set suggest that the proposed two models are effective and outperform baselines in most settings. This report extends the paper "Correlated Time Series Forecasting using Multi-Task Deep Neural Networks," to appear in ACM CIKM 2018, by providing additional experimental results.

==> ForNextMeeting.tex <==
1 Scalar Saga

Hi,

Regarding the scaling of data for the models:
We initially tried to remove the scalar completely, but we then realized that some of the models final output node have a sigmoid activation function and so we need a method getting from the range (0;1) to the target values, but since we don't have a scalar we can not do it. 
There is a function that reverses sigmoid but due to limited number of floating points decimals it tops out at a specific value.
For the moment, 









Question #1:

Charts representation

We were wondering about what charts would best present our results.
We are aiming to show 3 assumptions

1 Linear vs non linear

Here we test the assumption that no linear algorithms can outperform linear ones. We have two linear algorithms, both univariate (ARIMA and yesterday).
For a fair comparison, we can only use the the univariate versions of the other algorithms, or also include the multivariate ones.

The graph can look as follows:

This graphs show the results for all algorithms for 1 part of 1 data set. This can means we can have up to 18 (6 chemical thanks * 3 sections data per tank) of these graphs. We can run an average on all sewage data sets and sections and reduce them to 1 of these graphs. We can also indicate standard deviation per each data set if we average.




2 Univariate vs multivariate

For this one we can use bar charts to compare error scores for each algorithms with 2 and 1 (-S) time series. Also it will compare overall. It would look something like this. We can also add a third one

We also want to show that adding a random time series (-R) (uncorrelated) runs as bad as running a univariate (-S) model (or at least not much worse). This checks the initial assumption that the time series in the input set contain correlated time series.

This graphs show the results for all algorithms for 1 part of 1 data set. This can means we can have up to 18 (6 chemical thanks * 3 sections data per tank) of these graphs. We can run an average on all sewage data sets and sections and reduce them to 1 of these graphs. We can also indicate standard deviation per each data set if we average.


3 How our algorithms outperforms its competitors

for this we believe a line chart would be proper. One line for each algorithm connecting value for error on Y axes and different combinations of parameter on the X axes. The following is basic representation.

Again we can try to average out the sewage data sets and also use standard deviation.

For all the graphs presented up-top we can show the per data set errors within tables together with the averages presented in the charts.


Question #2:

Regarding standard deviation.

In the previous question we talked about averaging the error scores over the sewage data sets and showing the standard deviation how much deviation there is from this average. Is this a proper use of the standard deviation or are we misunderstanding it?


Question #3:

Regarding the adjustments of the experiments hyper parameters.

For proper results things like learning rate (each model has its own values) have to be adjusted for each data set we use; but this is not feasible. In contrast we are thinking of setting parameters for each combination of problem parameters (n, l, p).

Question #4:

Overall number and duration of the experiments.

In this excel we present how changing the number of parameters effects the estimated running time of the whole experimental setup.

https://docs.google.com/spreadsheets/d/1a1jhzLn3-8V9aZxrRVez1wFaWPJGec7cWSqR5bTROLU/edit#gid=0

For each of the 6 aeration tanks we can take 3 different sets of data (Parts from sewage data) 6*3=18. We then adjust the problem parameters l (size of model input) p (prediction window; size of model output) n (number of time series) 3 + 4 + 2 = 9. We do this for each of the 7 algorithms for a final 18*9*7 = 1134 execution of each algorithm.

From running the experiments we realized that an average run takes around 7 minutes (including all the adjustments for hyper parameters). Thus we have 7938 minutes run time for the sewage data set alone 132 hours.

Adding two more data sets from google trends we have an addition 2*9*7*7 = 882 minutes.

For a total of 8820 minutes or 147 hours, we believe this to be way too much time to be feasible.

Were could we possible reduce the running time, or how could we avoid running so many tests.



==> ideas.tex <==
A)Modular neural network

O colectie de nn care lucreaza indepndent dupa care rezultatul lor e combinat intr-un alt nn sa iasa predictia.

Input: un array de length 60/100/200 2 ts (30/50/100 fiecare)

Output: 20,25 step predictions for first time series

Putem incerca

1

doua CNN ca independent nn
fiecare primeste cate 1 (si doar 1) din ts
cum un TS are o singura dimensiune nu stiu exact cum va merge.

contine un convolutional 
si un pooling layer reduci la 15/25/50 (50\% daca nu e prea mult, sau cum se face pooling)

rezultatul (din pooling layers) celor 2 CNN sa fie combinat

1a fie tot intr-un CNN care sa dea predictia
1b fie intru nn cu node si activation sa dea...
1c LSTM/RNN

2

doua regular node+activation function NN 
aceasi idei


B) Idea lui gabi

Antenat mai multe NN (FFNN CNN sau LSTM) sa prezica doar o componenta din final rezult, combine everything into a final rezult.

Input: un array de lenght 60/100/20 2 ts (30/50/100 fiecare)
NN iau acelasi input mereu.

Output fiecare NN va genera o parte din output

Fiecare NN va invata sa genereze o parte din ouput size 1/n (n fiinde cate NN) 0 1/n 2/n.. n-1/n steps ahead.



Test if given an correlated time series it takes the performance worse.

==> sections/figures/Single_Correlated_Random.tex <==
\begin{tabular}{lll}
\hline
 Config/Alg   & MCRNN        & MAECNNRNN    \\
\hline
 Single       & \text{10.75} & \text{10.72} \\
 Correlated   & \text{8.29}  & \text{9.06}  \\
 Random       & \text{13.02} & \text{10.71} \\
\hline
\end{tabular}

==> sections/future_work.tex <==
\section{Future work}
\label{future_work}


